FEDMEKI: A Benchmark for Scaling Medical Foundation Models via Federated Knowledge Injection

This study introduces the Federated Medical Knowledge Injection (FEDMEKI) platform, a new benchmark designed to address the unique challenges of integrating medical knowledge into foundation models under privacy constraints. By leveraging a cross-silo federated learning approach, FEDMEKI circumvents the issues associated with centralized data collection, which is often prohibited under health regulations like the Health Insurance Portability and Accountability Act (HIPAA) in the USA. The platform is meticulously designed to handle multi-site, multi-modal, and multi-task medical data, which includes 7 medical modalities, including images, signals, texts, laboratory test results, vital signs, input variables, and output variables. The curated dataset to validate FEDMEKI covers 8 medical tasks, including 6 classification tasks (lung opacity detection, COVID-19 detection, electrocardiogram (ECG) abnormal detection, mortality prediction, sepsis prediction, and enlarged cardiomediastinum detection) and 2 generation tasks (medical visual question answering (MedVQA) and ECG noise clarification). This comprehensive dataset is partitioned across several clients to facilitate the decentralized training process under 16 benchmark approaches. FEDMEKI not only preserves data privacy but also enhances the capability of medical foundation models by allowing them to learn from a broader spectrum of medical knowledge without direct data exposure, thereby setting a new benchmark in the application of foundation models within the healthcare sector.

==> section/app-CaseStudy.tex <==
\section{Case Study}

\subsection{RSNA Pneumonia Detection}

\subsection{ECG Abnormal Detection}

\subsection{Mortality Prediction}

\subsection{MedQA}


\subsection{MedVQA}

\subsection{Covid Detection}

\subsection{Sepsis Prediction}

==> section/app-MedQA.tex <==
% \section{Training Task -- MedQA (no need)}\label{app:medqa}

% \subsection{Description}

% \subsection{License and Ethics}

% \subsection{Access and Preprocessing}

% This task, based on a widely-adopted data source~\cite{zhang2018medical}, requires the model to provide correct textual answer based on a medical context description. The dataset is publicly accessible at \footnote{https://drive.google.com/file/d/1ImYUSLk9JbgHXOemfvyiDiirluZHPeQw/view}.

% \subsection{Task}

% \subsection{Data Samples}

% \subsection{Data Split}

% \subsection{Loss Function}

==> section/benchmark.tex <==
\section{Benchmark}

In this section, we first outline the experimental setups (Sec. \ref{sec:setups}). We then detail the formulation of the uni-task benchmark (Sec. \ref{sec:uni-task}), multi-task benchmark (\ref{sec:multi-task}) as well as the transfer learning benchmark (\ref{sec:transfer_learning}). 
% \Additionally, we provide an experimental analysis of {\model} (Sec. \ref{sec:study_on_ours})to gain insights into developing subsequent knowledge injection approaches for medical foundation models.



\subsection{Experiment Setups}
\label{sec:setups}
% \noindent\textbf{Setting}
% \begin{itemize}
%     \item What datasets?
%     \item How many tasks we consider?
%     \item What models we use for the clients and the foundation model?
% \end{itemize}




% \noindent\textbf{Tasks \& Datasets}
% \begin{itemize}
%     \item Image Classification: RSNA%, CheXpert, Covid-19
%     % \item Image Segmentation:  BRATS%, LiTS, KiTS 
%     \item Criticality Prediction: MIMIC-III%, eICU
%     \item ICD Coding: MIMIC-III
%     \item MedQA: MedQA
% \end{itemize}

% We can also cover few-show learning, but need to think about baselines first. (Or cover these experiments as additional study.)

% \noindent\textbf{Client Models}
% \begin{itemize}
%     \item Image Classification: CNN
%     % \item Image Segmentation:  CNN
%     \item Criticality Prediction: LSTM
%     \item ICD Coding: LSTM
% \end{itemize}



\noindent\textbf{Baselines} We include the following baselines in our benchmark. These baselines are common strategies of developing medical models under the data privacy constraint.

\begin{itemize}

    \item \textbf{Fine-tuning(FT)}: This approach utilizes only the minority of the training data with the foundation model \xiaochen{or local model?} in a centralized manner, representing scenarios where only limited public health data are accessible. It mirrors real-world situations where researchers focusing on healthcare foundation model merely rely on limited public data due to privacy concerns or regulatory restrictions.
    \item \textbf{Federated Learning (FL)}: This method involves the majority of the training data being distributed across clients, each training a local model within their own private domain. These local models engage in conventional Federated Learning approaches, e.g., FedAVG, to produce a global model. This setting represents scenarios in which numerous health institutions utilize their specific but scattered medical data to develop targeted models. These institutions may lack the computational resources to develop large, powerful foundation models, hence they leverage federated learning to optimize task-specific models training across decentralized data sources while maintaining data privacy and locality.
    \item \textbf{Federated Learning + Fine-tuning (FL-FT)}: This approach extends traditional federated learning processes by incorporating an additional training phase on the server. After constructing task-specific model through the aggregation of local models trained on dominant private client data, the resulted model is further fine-tuned with scarce publicly available data. This approach benefits from both private and public medical data, but without involvement of foundation model. 
    \item \textbf{Centralized FT (CFT)}: This method utilizes 100\% of the training data with the foundation model deployed on the server, simulating an ideal yet impossible scenario where all medical data are available centrally without any distribution constraints.
\end{itemize}

\noindent\textbf{Evaluation Metric} We utilize accuracy, precision, recall, F1, and MCC for assessment on classification tasks, while BLEU, ROUGE1, and METEOR serve as evaluation metrics for the generative task.


\noindent\textbf{Implementation}
 We adopt the cross-silo setting and configured five clients per task, with the number of communication rounds set at 10 We initialize the foundation model with a MMedLM 2 \cite{qiu2024towards} checkpoint. We adopt the Parameter-efficient Fine-tuning (PEFT) strategy for training the foundation model, which means that parameters in transformer layers are frozen during gradient backpropagation. Encoders employed for each modalities are listed in Table \ref{tab:encoder}. 

\noindent\textbf{Data Preprocessing} To reduce the heterogeneity of different datasets and data types, we standardize the data used in the benchmark by transforming all of it into a question-answering format. A template of the standardized output can be found in the Appendix.

\noindent\textbf{Data Distribution:} To emulate the real-world distribution of decentralized medical data, we allocated the majority of the data, 70\%, for each task across the clients. A minority, 10\%, was retained on the server. The remaining 20\% of the data was used as the validation and test set, splitting with the ratio 1:1.

\begin{table}[]
\begin{tabular}{l|l|l}
\hline
Modality          & Encoder         & \# of parameters \\ \hline
Text              & Embedding Layer &  379M                                  \\
Image             & Deit-Tiny\cite{touvron2021training}       &  8M                                  \\
Signal               & LSTM            & 1M                                   \\
Temporal Readings & LSTM            &                                    \\
Demographics      & MLP             &                                    \\ \hline
\end{tabular}
\caption{Encoders for each modality.}
\label{tab:encoder}
\end{table}

% \subsection{Expansibility Experiment Settings}

% Zero-shot Learning: Undertake new task, compare with model not trained on relevant tasks. Encoders on clients are well-trained.
% \begin{itemize}
    
%     \item Same Modality - New Task: Training on shock prediction and evaluating on mortality prediction.
%     \item New Modality Combination - New Task: Training on QA and image classification, evaluating on VQA.
    
% \end{itemize}

% Few-shot Learning: Undertake new task, compare with model not trained on relevant tasks. Encoders on clients are well-trained.
% \begin{itemize}
    
%     \item Same Modality - New Task: Well-training on shock prediction, and few-shot learning + evaluating on mortality prediction.
%     \item New Modality Combination - New Task: Well-training on QA and image classification, few-shot learning + evaluating on VQA.
%     \item New Individual Modality - New Task: Well-training on med-QA, few-shot learning + evaluating on image classification. (not sure if it can work.)
    
% \end{itemize}


\subsection{Uni-task Benchmark}
\label{sec:uni-task}
Medical foundation models, enhanced through targeted knowledge injection, are expected to perform specific tasks effectively upon activation. To assess the degree to which these models leverage knowledge injection for particular tasks, we introduce a uni-task benchmark. In this benchmark, models are trained exclusively on a single dataset and subsequently evaluated on its corresponding test set. Experimental results are presented in Table \ref{tab:unitask}



% \begin{table}[ht]
% \centering
% \tiny
% \caption{Uni-task Benchmark}
% \label{tab:unitask}
% \begin{tabular}{l|l|l|l|l}
% \hline
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{1}{c|}{\textbf{Lung Opacity Detection}} & \multicolumn{1}{c|}{\textbf{MedQA}} & \multicolumn{1}{c|}{\textbf{Signal QA}} & \multicolumn{1}{c}{\textbf{Shock Prediction}} \\ \cline{2-5}
%                                   & RSNA                     & MedQA          & ECG-QA            & MIMIC-III                         \\ \hline
% Public Training                   & 90.31                         &  45.04              &                   &                                   \\ \hline
% Private Training                  & 90.14                         & 0.45               &                   &                                   \\ \hline
% Centralize Training               & 93.35                         & 53.92               &                   &                                   \\ \hline
% Collaborative Training            & 91.61                         & 2.35               &                   &                                   \\ \hline
% {\model}                          & 90.71                         & 43.91               &                   &                                   \\ \hline
% \end{tabular}
% \end{table}


\begin{table}[ht]
\centering
\tiny
\caption{Uni-task Benchmark}
\label{tab:unitask}
\begin{tabular}{l|l|cccc|ccc|cccc|cccc}
\hline
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Clients}} & \multicolumn{4}{c|}{\textbf{Lung Opacity}} & \multicolumn{3}{c|}{\textbf{MedQA}} & \multicolumn{4}{c|}{\textbf{Abnormal Signal Detection}} & \multicolumn{4}{c}{\textbf{Mortality Prediction}} \\ \cline{3-17}
                                 &                      & ACC & Prec. & Recall & F1 & BLEU & R1 & MET. & ACC & Prec. & Recall & F1 & ACC & Prec. & Recall & F1 \\ \hline
CFT                               & 0 & 93.35 &  &  &  & 53.92 & 55.79 & 47.43 &  &  &  &  &  &  &  &  \\ \hline
FT                               & 0 & 87.41 & 86.88 & 89.17 & 88.01 & 45.04 & 47.53 & 39.77 &  &  &  &  &  &  &  &  \\ \hline
FL                            & 3 & 92.10 & 95.80 & 88.64 & 92.08 & 0.45 &  &  & 64.37 & 75.05 & 58.51 & 65.76 &  &  &  &  \\ \cline{2-17}
                                 & 5 & 89.16 & 99.09 & 79.81 & 88.41 & 2.35 & 4.69 & 13.72  & 58.92 & 60.55 & 85.33 & 70.83 &  &  &  &  \\ \cline{2-17}
                                 & 10 & 86.55 & 95.95 & 77.29 & 85.61 & 2.35 & 4.67 & 13.63  & 58.41 & 58.45 & 99.84 & 73.73 &  &  &  &  \\ \hline
FL + FT                          & 3 & 90.74 & 94.94 & 86.75 & 90.66 & 2.40 & 4.81 & 14.24 & 66.21 & 71.05 & 71.22 & 71.13 &  &  &  &  \\ \cline{2-17}
                                 & 5 & 88.07 & 96.33  & 80.02 & 87.42 & 2.35 & 4.69 & 13.72 & 60.39 & 62.95 & 78.35 & 69.81 &  &  &  &  \\ \cline{2-17}
                                 & 10 & 87.58 & 89.17 & 86.54 & 87.83 & 2.35 & 4.67 & 13.63 & 57.08 & 60.43 & 77.02 & 67.72 &  &  &  &  \\ \hline
\model                           & 3 & 90.71 &  &  &  & 43.91 &  &  &  &  &  &  &  &  &  &  \\ \cline{2-17}
                                 & 5 & 92.21 & 90.40 & 95.05 & 92.67 & 43.91 & 46.04 & 38.46 &  &  &  &  &  &  &  &  \\ \cline{2-17}
                                 & 10 & 90.71 &  &  &  & 43.91 &  &  &  &  &  &  &  &  &  &  \\ \hline
\end{tabular}
\end{table}

\noindent\textbf{Task Expandability Test}
Using model trained on task 1 modality A to do few shot learning on task 2 modality A.


\noindent\textbf{Modality Expandability Test}
Using model trained on task 1 modality A to do few shot learning on task 1 modality B. (QA vs VQA)

\noindent\textbf{QA Test}
Compare {\model} with original MMedLM2 on MEDQA task to prove that injection works.


% \noindent\textbf{Unimodal Evaluation}

% The evaluation results on unimodal tasks are listed in Table \ref{tab:unimodal_tasks_comparison}. \xiaochen{Analysis to be provided}. 

% \begin{table}[ht]
% \centering
% \tiny
% \begin{tabular}{l|l|l|l|l|l|l|l}
% \hline
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{Image Classification}} & \multicolumn{2}{c|}{\textbf{Covid Detection}} & \textbf{Cardiomediastinum} & \textbf{ICD Coding} & \textbf{Medical Question Answering} \\ \cline{2-8} 
%                                   & RSNA                       & CheXpert                & Covid-19                 & CoughVID                & CheXpert                & MIMIC-III           & MedQA                          \\ \hline
% Centralized Training                         &                            &                         &                          &                         &                         &                                    &                             \\ \hline
% Public Training                         &                                                &                          &                         &                         &                     &                 &                             \\ \hline
% Private Training                         &                                               &                          &                         &                         &                     &                 &                             \\ \hline
% {\model}                         &                                                &                          &                         &                         &                     &                 &                             \\ \hline
% \end{tabular}
% \label{tab:unimodal_tasks_comparison}
% \caption{Benchmark on Unimodal Healthcare Tasks}
% \end{table}


% \noindent\textbf{Multimodal Evaluation}

% The experiment results on multimodal tasks are listed in Table \ref{tab:multimodal_tasks_comparison}. \xiaochen{Analysis to be provided}. 

% \begin{table}[ht]
% \centering
% \tiny
% \label{tab:multimodal_tasks_comparison}
% \begin{tabular}{l|l|l|l|l|l|l|l|l}
% \hline
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{ARF Prediction}} & \multicolumn{2}{c|}{\textbf{Shock Prediction}} & \multicolumn{2}{c|}{\textbf{Mortality Prediction (valid)}} & \multicolumn{2}{c}{\textbf{Medical Image Captioning}} \\ \cline{2-9} 
%                                   & MIMIC-III               & eICU                & MIMIC-III                 & eICU                 & MIMIC-III                                & eICU                             & CheXpert                 & OpenI               \\ \hline
% Centralized Training                                &                         &                     &                           &                      &                                          &                                  &                          &                      \\ \hline
% Public Training                         &                         &                     &                           &                      &                                          &                                  &                          &                      \\ \hline
% Private Training                           &                         &                     &                           &                      &                                          &                                  &                          &                      \\ \hline

% {\model}                        &                         &                     &                           &                      &                                          &                                  &                          &                      \\ \hline
% \end{tabular}
% \caption{Comparison of Methods for Multimodal Tasks}
% \end{table}

\subsection{Multi-task Benchmark}
\label{sec:multi-task}

In the uni-task benchmark, knowledge injection approaches are examined with individual task. In addition to evaluation per task, assessing how model benefits from knowledge in other tasks becomes equivalently essential for comprehensively evaluation, as real-world foundation models are usually trained with diverse tasks. Hence, we design the multitask benchmark. In this suite of experiments, models are trained on all tasks beforehand rather than single ones, meaning that knowledge from a wider spectrum is injected to them. The performances of fully-trained models are listed in Table \ref{tab:multitask}

\begin{table}[ht]
\centering
\tiny
\caption{Multi-task Benchmark}
\label{tab:multitask}
\begin{tabular}{l|l|l|l|l}
\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{1}{c|}{\textbf{Lung Opacity Detection}} & \multicolumn{1}{c|}{\textbf{MedQA}} & \multicolumn{1}{c|}{\textbf{Signal QA}} & \multicolumn{1}{c}{\textbf{Shock Prediction}} \\ \cline{2-5}
                                  & RSNA                     & MedQA          & ECG-QA            & MIMIC-III                         \\ \hline
Public Training                   &                          &                &                   &                                   \\ \hline
Private Training                  &                          &                &                   &                                   \\ \hline
Centralize Training               &                          &                &                   &                                   \\ \hline
Collaborative Training            &                          &                &                   &                                   \\ \hline
{\model}                          &                          &                &                   &                                   \\ \hline
\end{tabular}
\end{table}



\subsection{Low-resource Learning Benchmark}
\label{sec:transfer_learning}
As forecasted in previous work \cite{moor2023foundation}, ideal medical foundation models should possess a robust capability to handle unseen tasks. Correspondingly, an effective knowledge injection approach should enable the targeted model to establish connections between encountered and unseen tasks, thereby demonstrating a commendable ability to manage the latter. To evaluate this critical characteristic of knowledge injection approaches, we propose the Low-resource Learning Benchmark. The fully-trained foundation model, as detailed in Section \ref{sec:multi-task}, is assessed on unseen tasks with no or minimal data available, employing zero- and few-shot learning settings. The benchmark is provided in Table \ref{tab:low_resource}.




\begin{table}[ht]
\centering
\tiny
\caption{Low-resource Learning Benchmark}
\label{tab:low_resource}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{1}{c|}{\textbf{Covid Detection}} & \multicolumn{1}{c|}{\textbf{ARF Prediction}} & \multicolumn{1}{c|}{\textbf{Cardiomediastinum Prediction}} & \multicolumn{1}{c|}{\textbf{Sleep Apnea Detection}} & \multicolumn{1}{c|}{\textbf{Mortality Prediction}} & \multicolumn{1}{c}{\textbf{MedVQA}} \\ \cline{2-7} 
                                  & Covid-19             & MIMIC-III          & CheXpert                           & MIT-BIH                       & MIMIC-III                    & RAD                      \\ \hline
Public Training                   &                       &                    &                                    &                               &                              &                          \\ \hline
Private Training                  &                       &                    &                                    &                               &                              &                          \\ \hline
Centralize Training               &                       &                    &                                    &                               &                              &                          \\ \hline
Collaborative Training            &                       &                    &                                    &                               &                              &                          \\ \hline
{\model}                          &                       &                    &                                    &                               &                              &                          \\ \hline
\end{tabular}
\end{table}




% \subsection{Study on {\model}}

% To provide insights on the design of {\model}, we conduct the following experiments, comparing {\model} with PEFT counterparts. We select the task of lung opacity detection and MedQA as representatives of learned tasks, while MedVQA serves as the unseen tasks. Baselines and {\model} are trained on tasks of lung opacity detection and MedQA, then evaluated on all three tasks. The results can be found in Table \ref{tab:model_study}.

% \begin{table}[ht]
% \centering
% \tiny
% \caption{Study on {\model}}
% \label{tab:model_study}
% \begin{tabular}{l|l|l|l}
% \hline
% \textbf{Method} & \textbf{Lung Opacity Detection} & \textbf{MedQA} & \textbf{MedVQA} \\ \hline
% Octavius\cite{chen2023octavius}        &                                       &                 &                              \\ \hline
% Lavin\cite{luo2024cheap}           &                                       &                 &                              \\ \hline
% {\model}        &                                       &                 &                              \\ \hline
% \end{tabular}
% \end{table}


% \label{sec:study_on_ours}

==> section/experiments.tex <==
\section{Benchmark}

\subsection{Data Partition}

We divide the data into two sets: training tasks and testing tasks, and there are \textbf{no overlaps} between the two kinds of tasks.


The \textbf{training tasks} include XXX. We can observe that the training tasks consist of XXX modalities. 
For each training task, we keep 10\% data as public data denoted as $\mathcal{D}_p^{tra}$, XX\% as validation data $\mathcal{D}_{v}^{tra}$, and the remaining XX\% data $\mathcal{D}_{t}^{tra}$ are evenly distributed to 5 clients.

The \textbf{testing tasks} aim to evaluate the capability of zero-shot and few-shot learning, including XXX, XXX, and XXX tasks. For each testing task, we use XX data $\mathcal{D}_{p}^{test}$ for the few-shot fine-tuning and the remaining XX data $\mathcal{D}_{v}^{test}$ for the real testing. 

\subsection{Approaches}

We use the following approaches as benchmarks for the evaluation of \textbf{training tasks}, which will be evaluated with the validation data of the training tasks, i.e., $\mathcal{D}_{v}^{tra}$.

\textbf{LLM only}. The LLM used in this work is MMedLM-2, which can only input text data. Thus, only text modality-based tasks can have results. We use $\text{MMedLM}_{zero}$ denote the zero-shot inference and $\text{MMedLM}_{fs}$ represent the few-shot learning, where $\text{MMedLM}_{fs}$ is fine-tuned using the public data $\mathcal{D}_p^{tra}$ of training tasks.

\textbf{Traditional Federated Learning} (TFL). We use two representative federated learning models as benchmark baselines: FedAvg and FedProx. We consider two scenarios: (1) single-task federated learning and (2) multi-task federated learning. The single-task federated learning uses a task-specific dataset to train an individual \textbf{FedAvg}$_{s}$ or \textbf{FedProx}$_{s}$ model. The multi-task federated learning aims to place a multi-task model for each client, which is denoted as \textbf{FedAvg}$_{m}$ or \textbf{FedProx}$_{m}$. In such a way, all tasks can be trained together. The client-level multi-task model is the same as that of {\model}. Note that single-task federated learning and multi-task federated learning models will perform the same if no training tasks use multiple modalities as input.

\textbf{Federated Learning with Global Fine-tuning} (FL+GF). Since the server stores a small set of public data $\mathcal{D}_p^{tra}$, the traditional models can conduct the fine-tuning using $\mathcal{D}_p^{tra}$ for the aggregated global models. These approaches are denoted as \textbf{FedAvg}$^{+}_{s}$, \textbf{FedAvg}$^{+}_{m}$, \textbf{FedProx}$^{+}_{s}$, and \textbf{FedProx}$^{+}_{m}$, respectively.

\textbf{Federated Learning with LLM Fine-tuning} (FL+LLM). To further enhance the learning ability of traditional federated learning approaches, we allow them to fine-tune with the LLM, which can be treated as simplified versions of {\model}. In particular, the encoder of each aggregated model will be used first to generate the representation of the public data. The representation is then concatenated with the representation of LLM to generate the output. We denote these LLM fine-tuning approaches as \textbf{FedAvg}$^{\mathcal{F}}_{s}$, \textbf{FedAvg}$^{\mathcal{F}}_{m}$, \textbf{FedProx}$^{\mathcal{F}}_{s}$, and \textbf{FedProx}$^{\mathcal{F}}_{m}$, respectively.

\textbf{Federated Multi-task Fine-tuning} (FMF). The proposed {\model} is a federated multi-task fine-tuning framework, which allows the LLM to scale its capability to handle new tasks by injecting knowledge from federated clients. Based on the different ways to aggregate client encoders, we can have two variants of {\model}, i.e., \model$_{Avg}$ and  \model$_{Prox}$.




For the evaluation of \textbf{testing tasks}, we will compare the proposed {\model} against the original MMedLM under both zero-shot and few-shot learning scenarios. Similarly, only tasks with text as the input can make comparisons. For other tasks, MMedLM does not work at all. Let \model$^{zero}_{Avg}$/\model$^{zero}_{Prox}$ and \model$^{fs}_{Avg}$/\model$^{fs}_{Prox}$ denote the zero-shot and few-shot learning models, where \model$^{fs}$ uses $\mathcal{D}_{p}^{test}$ to do the fine-tuning. These models are evaluated on $\mathcal{D}_{v}^{test}$. These approaches are summarized in Table~\ref{tab:all_approaches}.

\begin{table}[t]
    \centering
    \caption{Summary of all benchmark approaches.}
    \label{tab:all_approaches}
\resizebox{1\textwidth}{!}
{
    \begin{tabular}{c|c|l|c|l|l|c}
    \hline
     \textbf{Setting }   &  \textbf{Category} &   \textbf{Model Name} & \textbf{LLM} & \textbf{Client Data} & \textbf{Server Data} & \textbf{Validation}\\\hline
     \multirow{16}{*}{\rotatebox[origin=c]{90}{Training Tasks}}   
     & \multirow{2}{*}{LLM Only }
      & MMedLM$_{zero}$ & \checkmark & \xmark & \xmark & \multirow{16}{*}{$\mathcal{D}_{v}^{tra}$}\\\cline{3-6}
     && MMedLM$_{fs}$ & \checkmark &\xmark & $\mathcal{D}_{p}^{tra}$ of a single task&\\\cline{2-6}
     
     & \multirow{4}{*}{TFL}
     & FedAvg$_{s}$ & \xmark& $\mathcal{D}_{t}^{tra}$ of a single task & \xmark &\\ \cline{3-6}
     && FedProx$_{s}$ & \xmark&$\mathcal{D}_{t}^{tra}$ of a single task & \xmark &\\ \cline{3-6}
     && FedAvg$_{m}$ & \xmark&$\mathcal{D}_{t}^{tra}$ of all tasks & \xmark &\\ \cline{3-6}
     && FedProx$_{m}$ & \xmark&$\mathcal{D}_{t}^{tra}$ of all tasks & \xmark &\\\cline{2-6}

     & \multirow{4}{*}{FL+GF}
     & FedAvg$_{s}^+$ & \xmark&$\mathcal{D}_{t}^{tra}$ of a single task & $\mathcal{D}_{p}^{tra}$ of a single task &\\ \cline{3-6}
     && FedProx$_{s}^+$ & \xmark&$\mathcal{D}_{t}^{tra}$ of a single task & $\mathcal{D}_{p}^{tra}$ of a single task &\\ \cline{3-6}
     && FedAvg$_{m}^+$ & \xmark&$\mathcal{D}_{t}^{tra}$ of all tasks & $\mathcal{D}_{p}^{tra}$ of all tasks & \\\cline{3-6}
     && FedProx$_{m}^+$ & \xmark&$\mathcal{D}_{t}^{tra}$ of all tasks & $\mathcal{D}_{p}^{tra}$ of all tasks &\\\cline{2-6}

     & \multirow{4}{*}{FL+LLM}
     & FedAvg$_{s}^{\mathcal{F}}$ & \checkmark &$\mathcal{D}_{t}^{tra}$ of a single task & $\mathcal{D}_{p}^{tra}$ of a single task &\\ \cline{3-6}
     && FedProx$_{s}^{\mathcal{F}}$ & \checkmark &$\mathcal{D}_{t}^{tra}$ of a single task & $\mathcal{D}_{p}^{tra}$ of a single task &\\ \cline{3-6}
     && FedAvg$_{m}^{\mathcal{F}}$ & \checkmark &$\mathcal{D}_{t}^{tra}$ of all tasks & $\mathcal{D}_{p}^{tra}$ of all tasks & \\\cline{3-6}
     && FedProx$_{m}^{\mathcal{F}}$ & \checkmark &$\mathcal{D}_{t}^{tra}$ of all tasks & $\mathcal{D}_{p}^{tra}$ of all tasks &\\\cline{2-6}

     & \multirow{2}{*}{FMF}
     & \model$_{Avg}$ & \checkmark &$\mathcal{D}_{t}^{tra}$ of all tasks & $\mathcal{D}_{p}^{tra}$ of all tasks &\\\cline{3-6}
     &&\model$_{Prox}$ & \checkmark &$\mathcal{D}_{t}^{tra}$ of all tasks & $\mathcal{D}_{p}^{tra}$ of all tasks &\\\hline\hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{Testing Tasks}}   
     & \multirow{3}{*}{Zero-shot }
      & MMedLM$_{zero}$ & \checkmark & \xmark & \xmark & \multirow{6}{*}{$\mathcal{D}_v^{test}$}\\\cline{3-6}
      && \model$_{Avg}^{zero}$ & \checkmark & \xmark & \xmark &\\\cline{3-6}
     && \model$_{Prox}^{zero}$ & \checkmark & \xmark & \xmark &\\\cline{2-6}

     & \multirow{3}{*}{Few-shot }
     & MMedLM$_{fs}$ & \checkmark & \xmark & $\mathcal{D}_p^{test}$ of a single task &\\\cline{3-6}
     
     && \model$_{Avg}^{fs}$ & \checkmark & \xmark & $\mathcal{D}_p^{test}$ of all tasks &\\\cline{3-6}
     && \model$_{Prox}^{fs}$ & \checkmark & \xmark & $\mathcal{D}_p^{test}$ of all tasks &\\\hline

    \end{tabular}
}
\end{table}




\begin{table}[t]
    \centering
    \caption{Summary of Model Performance on Various Tasks.}
    \label{tab:model_performance}
\resizebox{1\textwidth}{!}
{
    \begin{tabular}{c|cccc|ccc|cccc|ccc|cccc}
    \hline
    \multirow{2}{*}{\textbf{Model Name}} & \multicolumn{4}{c|}{\textbf{Lung Opacity}} & \multicolumn{3}{c|}{\textbf{MedQA}} & \multicolumn{4}{c|}{\textbf{ECG Abnormal Detection}} & \multicolumn{3}{c|}{\textbf{ECGQA}} & \multicolumn{4}{c}{\textbf{Mortality Prediction}} \\ \cline{2-20}
    & \textbf{ACC} & \textbf{Prec.} & \textbf{Recall} & \textbf{F1} & \textbf{BLEU} & \textbf{R1} & \textbf{MET.} & \textbf{ACC} & \textbf{Prec.} & \textbf{Recall} & \textbf{F1} & \textbf{BLEU} & \textbf{R1} & \textbf{MET.} & \textbf{ACC} & \textbf{Prec.} & \textbf{Recall} & \textbf{F1} \\ \hline
    MMedLM$_{zero}$ & \xmark & \xmark & \xmark & \xmark & - & - & - & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark &\xmark & \xmark & \xmark & \xmark \\ \hline
    MMedLM$_{fs}$ & \xmark & \xmark & \xmark & \xmark & - & - & - & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark &\xmark & \xmark & \xmark & \xmark \\ \hline
    FedAvg$_{s}$ & 89.16 & 99.09 & 79.81 & 88.41 & 2.35 & 4.69 & 13.72  & 58.92 & 60.55 & 85.33 & 70.83 & - & - & - & - & - & - & - \\ \hline
    FedProx$_{s}$ & 93.41 & 95.11 & 92.01 & 93.53 & 0.00 & 4.41 & 12.75 & 45.62 & 67.45 & 13.49 & 22.48 & 0.00 & 0.00 & 0.00 & 91.74 & 76.92 & 3.11 & 5.97 \\ \hline
    FedAvg$_{m}$ & 85.13 & 96.82 & 73.71 & 83.70 & 0.00 & 4.42 & 12.86 & 71.25 & 79.14 & 69.02 & 73.73 & 0.00 & 0.00 & 0.00 & 91.66 & 83.33 & 1.55 & 3.05 \\ \hline
    FedProx$_{m}$ & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ \hline
    FedAvg$_{s}^+$ & 93.08 & 92.92  & 93.80 & 93.35 & 0.00 & 4.41 & 13.04 & 67.72 & 66.55 & 90.04 & 76.53 & 0.00 & 12.44 & 13.33 & 91.51 & 33.33 & 0.62 & 1.22 \\ \hline
    FedProx$_{s}^+$ & 89.49 & 87.90 & 92.43 & 90.11 & - & - & - & 60.84 & 68.26 & 61.73 & 64.83 & - & - & - & - & - & - & - \\ \hline
    FedAvg$_{m}^+$ & 93.08 & 92.92  & 93.80 & 93.93 & 2.37 & 4.71 & 13.95 & 67.72 & 66.55 & 90.04 & 76.53 & 0.00 & 12.44 & 13.33 & 91.56 & 0.00 & 0.00 & 0.00 \\ \hline
    FedProx$_{m}^+$ & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ \hline
    FedAvg$_{s}^{\mathcal{F}}$ & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ \hline
    FedProx$_{s}^{\mathcal{F}}$ & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ \hline
    FedAvg$_{m}^{\mathcal{F}}$ & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ \hline
    FedProx$_{m}^{\mathcal{F}}$ & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ \hline
    \model$_{Avg}$ & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ \hline
    \model$_{Prox}$ & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ \hline
    \end{tabular}
}
\end{table}


\begin{table}[t]
    \centering
    \caption{Summary of Model Performance on Various Test Tasks.}
    \label{tab:test_tasks_performance}
\resizebox{1\textwidth}{!}
{
    \begin{tabular}{c|ccc|cccc|cccc}
    \hline
    \multirow{2}{*}{\textbf{Model Name}} & \multicolumn{3}{c|}{\textbf{MedVQA}} & \multicolumn{4}{c|}{\textbf{Covid Detect}} & \multicolumn{4}{c}{\textbf{Sepsis}} \\ \cline{2-13}
    & \textbf{BLEU} & \textbf{R1} & \textbf{MET.} & \textbf{ACC} & \textbf{Prec.} & \textbf{Recall} & \textbf{F1} & \textbf{ACC} & \textbf{Prec.} & \textbf{Recall} & \textbf{F1} \\ \hline
    MMedLM$_{zero}$ & - & - & - & - & - & - & - & - & - & - & - \\ \hline
    \model$_{Avg}^{zero}$ & - & - & - & - & - & - & - & - & - & - & - \\ \hline
    \model$_{Prox}^{zero}$ & - & - & - & - & - & - & - & - & - & - & - \\ \hline
    MMedLM$_{fs}$ & - & - & - & - & - & - & - & - & - & - & - \\ \hline
    \model$_{Avg}^{fs}$ & - & - & - & - & - & - & - & - & - & - & - \\ \hline
    \model$_{Prox}^{fs}$ & - & - & - & - & - & - & - & - & - & - & - \\ \hline
    \end{tabular}
}
}
\end{table}


==> section/introduction.tex <==
% \section{Introduction}

% \xiaochen{Randomly written scratch.}

% Medical foundation models have become increasingly prevalent in medical applications due to their powerful capabilities. These models, conventionally, acquire knowledge through pretraining, which equips them with domain-specific knowledge and enables them to solve a subset of medical tasks. However, medical foundation models are highly constrained by their pretraining data, which are often limited to specific modalities, rendering them incapable of addressing tasks that require knowledge beyond the pretraining scope.

% To overcome this limitation, an ideal approach is to enrich the pretraining data. However, the nature of medical data—being highly scattered due to privacy issues and heterogeneous in terms of modalities—makes centralized training infeasible. General domain foundation models, such as \cite{}, can directly amass extensive volume of data for pre-training. Nevertheless, medical data cannot be consolidated without significant limitations.\xiaochen{Examples on privacy issue.}

% Therefore, we propose the medical knowledge injection task, wherein the medical foundation model is expected to acquire external knowledge from scattered, heterogeneous medical data without directly accessing this private data. To benchmark this task, we introduce {\model}, an initial approach for injecting knowledge into the medical foundation model. Our model gains external knowledge through federated encoding sharing and integrates this knowledge using parameter-efficient fine-tuning with a multitask multimodal mixture of experts module. The proposal of the medical knowledge injection problem, along with our initial benchmark, provides a solid foundation for future exploratory research in this domain.

% In summary, our main contributions are as follows:
% \begin{itemize}
%     \item \textit{Problem Formulation.} We clearly formulate the problem of injecting knowledge into Medical Foundation Models via federated learning.
%     \item \textit{{\model}.} We propose {\model}, an effective knowledge injection paradigm that enables federated medical foundation models to handle multiple tasks across diverse modalities, serving as an essential baseline for this challenge.
%     \item \textit{Open-sourced Experiment Environment.} We provide a standardized data preprocessing pipeline, a self-contained code repository, a reproducible benchmark, and in-depth analysis for further investigations into the development of medical foundation models.
% \end{itemize}


\section{Introduction}
\label{sec:intro}

Foundation models have revolutionized various domains by demonstrating powerful capabilities in handling different modalities and tasks. These models, such as GPT-3 and BERT in natural language processing, have shown exceptional performance across a wide range of applications. The primary reason for their success is their exposure to vast amounts of pretraining data, which allows them to acquire a deep understanding of diverse domains. By leveraging this extensive data, foundation models can generalize well and perform effectively on various tasks, making them invaluable in many fields.

In the medical domain, there have been attempts to develop medical foundation models to replicate the success seen in general domains. However, compared with counterpart in general domains, the development of these models is significantly hindered by the limited availability of public medical data. Collecting and aggregating sufficient medical data for pretraining these models sounds promising but is practically impossible due to stringent privacy regulations and ethical considerations. These constraints prevent the consolidation of medical data, impeding the progress in building robust medical foundation models.

Therefore, injecting knowledge into medical foundation models without directly sharing data becomes crucial. This approach allows models to benefit from the knowledge contained in distributed datasets while maintaining data privacy. The key challenge lies in effectively transferring and integrating this knowledge to enhance the foundation model's capabilities.

We define the process of medical knowledge injection into three important stages:

\noindent\textbf{Knowledge Extraction.} Effectively extracting high-quality medical knowledge from distributed models and scattered datasets is crucial. The accuracy and relevance of the distilled knowledge directly impact whether the foundation model gains valuable insights or merely noise. Ensuring the precision of this extraction process is vital for the overall performance of the model.

\noindent\textbf{Knowledge Transfer.} Transferring the extracted medical knowledge to the foundation model is an ongoing challenge. This process involves not only the physical transfer of data but also the integration of knowledge in a way that the model can utilize it effectively. Addressing the complexities of this transfer is essential for the seamless enhancement of the model.

\noindent\textbf{Knowledge Interiorization.} Even after extraction and transfer, external knowledge may not be immediately usable by the foundation model. Proper accommodation is necessary to embed this external knowledge into the medical foundation model effectively. This step ensures that the integrated knowledge aligns with the model's structure and enhances its capabilities.

Despite the importance of this problem, there isn't a clear benchmark for evaluating how medical models benefit from knowledge injection, nor is there a baseline. The absence of standardized evaluation criteria hampers the ability to measure progress and compare different approaches in this field.

Therefore, we propose the benchmark, {\model}. {\model} adopt a flexible design, allowing itself to take any type of medical modality to handle a variety of medical task. For the three stages mentioned before, {\model} uses local federated learning approach to extract healthcare knowledge from private data, shares encoders to transfer knowledge, and performs scaling on public data for effective knowledge integration. Our model gains external knowledge through federated encoding sharing and integrates this knowledge using parameter-efficient scaling with a multitask multimodal mixture of experts module. The proposal of the medical knowledge injection problem, along with our initial benchmark, provides a solid foundation for future exploratory research in this domain.

In summary, our main contributions are as follows:
\begin{itemize}
\item \textit{Problem Formulation.} We clearly formulate the problem of injecting knowledge into Medical Foundation Models via federated learning.
\item \textit{{\model}.} We propose {\model}, an effective knowledge injection paradigm that enables federated medical foundation models to handle multiple tasks across diverse modalities, serving as an essential baseline for this challenge.
\item \textit{Open-sourced Experiment Environment.} We provide a standardized data preprocessing pipeline, a self-contained code repository, a reproducible benchmark, and in-depth analysis for further investigations into the development of medical foundation models.
\end{itemize}

==> section/large_tables.tex <==
\begin{table}[ht]
\centering
\tiny
\caption{Uni-task Benchmark}
\label{tab:unitask}
\begin{tabular}{l|l|ccccc|ccc|ccccc|ccccc}
\hline
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Clients}} & \multicolumn{5}{c|}{\textbf{Lung Opacity}} & \multicolumn{3}{c|}{\textbf{MedQA}} & \multicolumn{5}{c|}{\textbf{Signal QA (ECG)}} & \multicolumn{5}{c}{\textbf{Shock Prediction (MIMIC)}} \\ \cline{3-20}
                                 &                      & ACC & Prec. & Recall & F1 & MCC & BLEU & R1 & MET. & ACC & Prec. & Recall & F1 & MCC & ACC & Prec. & Recall & F1 & MCC \\ \hline
CPT                               & 3 & 80.39 & 81.40 & 80.55 & 80.97 &  & 45.04 &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{2-20}
                                 & 5 & 90.31 &  &  &  &  & 45.04 &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{2-20}
                                 & 10 & 90.31 &  &  &  &  & 45.04 &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
PT                            & 3 & 89.81 & 98.35 & 81.70 & 89.26 & 0.80 & 0.45 &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{2-20}
                                 & 5 & 87.96 & 97.40 & 78.16 & 87.16 & 0.82 & 0.45 &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{2-20}
                                 & 10 & 90.96 & 96.78 & 85.38 & 90.73 & 0.83 & 0.45 &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
FL                               & 3 & 93.35 &  &  &  &  & 53.92 &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{2-20}
                                 & 5 & 89.81 & 98.35 & 81.70 & 91.45 &  & 53.92 &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{2-20}
                                 & 10 & 93.35 &  &  &  &  & 53.92 &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
FL+PT                          & 3 & 87.91  & 89.66 & 86.65 & 88.13 & 0.82 & 2.35 &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{2-20}
                                 & 5 & 87.51 & 97.48  & 77.18 & 86.15 & 0.77 & 2.35 &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{2-20}
                                 & 10 & 87.58 & 89.17 & 86.54 & 87.83 & 0.75 & 2.35 &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
\model                           & 3 & 80.39 & 81.40 & 80.55 & 80.97 &    & 43.91 &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{2-20}
                                 & 5 & 79.14 & 79.40 & 80.65 & 80.02 &  & 43.91 &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{2-20}
                                 & 10 & 81.80 & 88.23 & 74.69 & 81.00 &  & 43.91 &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
\end{tabular}
\end{table}


==> section/method_new.tex <==
\section{The proposed {\model} Framework}

\subsection{Framework Setups}

\textbf{Clients}. The goal of this work is to scale and enhance the predictive ability of medical large language models (LLMs) by incorporating medical knowledge from private client data in a federated manner. To achieve this, we employ $N$ clients, each representing a hospital or a medical institute holding private medical data $\mathcal{D}_n$. We assume that the private dataset $\mathcal{D}_n$ contains all medical modalities $\{\mathcal{M}_1, \cdots, \mathcal{M}_M\}$ and can perform all tasks $\{\mathcal{T}_1, \cdots, \mathcal{T}_T\}$. Each client trains a model $f_n = [\text{ENC}_n(); \text{DEC}_n()]$ using the data $\mathcal{D}_n$, where $\text{ENC}_n()$ is the encoder and $\text{DEC}_n()$ is the decoder/predictor. Thus, the model parameters $\boldsymbol{\theta}_n$ of $f_n$ can be divided into $\boldsymbol{\theta}_n^{enc}$ for the encoder and $\boldsymbol{\theta}_n^{dec}$ for the decoder, which will be further upload to the server.

\textbf{Server}. We deploy a generative medical foundation model, MMedLM-2\footnote{\url{https://huggingface.co/Henrychur/MMedLM2}}~\cite{qiu2024towards}, on the server, denoted as $\mathcal{F}$. MMedLM-2 is a state-of-the-art pre-trained medical language model that outperforms several LLMs on medical question-answering tasks. 
% Let $\text{ENC}_{\mathcal{F}}(\cdot;\boldsymbol{\varphi}_{\mathcal{F}}^{enc})$ and $\text{DEC}_{\mathcal{F}}(\cdot; \boldsymbol{\varphi}_{\mathcal{F}}^{dec})$ denote the encoder and decoder of $\mathcal{F}$, where $\boldsymbol{\varphi}_{\mathcal{F}}^{\cdot}$ denotes the corresponding parameters. The encoder $\text{ENC}_{\mathcal{F}}()$ encodes the input text $\mathcal{X}$ into a vector representation, i.e., $\mathbf{r}_{\mathcal{F}} = \text{ENC}_{\mathcal{F}}(\mathcal{X}; \boldsymbol{\varphi}_{\mathcal{F}}^{enc})$, while the decoder generates the response $\hat{\mathcal{Y}} = \text{DEC}_{\mathcal{F}}(\mathbf{r}_{\mathcal{F}}; \boldsymbol{\varphi}_{\mathcal{F}}^{dec})$.
We aim to inject medical knowledge represented by $\{\boldsymbol{\theta}_1^{enc}, \cdots, \boldsymbol{\theta}_N^{enc}\}$ into $\mathcal{F}$ and simultaneously update $\{\boldsymbol{\theta}_1^{enc}, \cdots, \boldsymbol{\theta}_N^{enc}\}$ by absorbing new knowledge from $\mathcal{F}$. These updated encoders and the aggregated decoders will then be distributed to the corresponding clients for learning in the next communication round. To facilitate the updates of client parameters, we place a small amount of public data on the server, denoted as $\mathcal{D}_p$.

Next, we provide client and server update details based on the previous setups.

\subsection{Client Updates -- Knowledge Extraction from Private Clients}
This benchmark framework allows each client to handle $T$ tasks simultaneously. Although these tasks have different training data, the modalities are partially shared, which motivates us to design a simple client model with $M$ modality-specific encoders and $T$ task-specific decoders. Table XXX lists the used encoders in the proposed framework.
We then use the following loss to train each client model:
\begin{gather}
    \min_{\boldsymbol{\theta}_n} \mathcal{L}_n := \frac{1}{T}\sum_{t=1}^T \frac{1}{|\mathcal{D}_n^t|} \sum_{(\mathbf{x}_i^t, \mathbf{y}_i^t) \in \mathcal{D}_n^t} \ell^t(f_n(\mathbf{x}_i^t; \boldsymbol{\theta}_n), \mathbf{y}_i^t),\\
    f_n(\mathbf{x}_i; \boldsymbol{\theta}_n) = \text{DEC}_{n,t}(\text{ENC}_{n,t}(\mathbf{x}_i; \boldsymbol{\theta}_{n,t}^{enc}); \boldsymbol{\theta}_{n,t}^{dec}),
\end{gather}
where $\mathcal{D}_n^t$ is the task-specific dataset, $\mathbf{x}_i^t$ and $\mathbf{y}_i^t$ are the data features and the corresponding ground truths, and $\ell^t$ is the loss function for a specific task, such as cross-entropy.
$\text{DEC}_{n,t}$ is the decoder for the $t$-th task with parameters $\boldsymbol{\theta}_{n,t}^{enc}$. $\text{ENC}_{n,t} \subseteq  \text{ENC}_n$ is the encoder for task $\mathcal{T}_t$ with parameters $\boldsymbol{\theta}_{n,t}^{dec}$, where $\text{ENC}_n=[\text{ENC}_n^1, \cdots, \text{ENC}_n^M]$ and $\text{ENC}_n^m$ denotes the encoder for the $m$-th modality.
The number of modality-level encoders in $\text{ENC}_{n,t}$ is determined by the input data. After the local training, we will upload the encoder and decoder parameters $\boldsymbol{\theta}_n^{enc}$ and $\boldsymbol{\theta}_n^{dec}$ to the server.


\subsection{Server Updates -- Knowledge Injection into Medical LLM}

\textbf{Knowledge Aggregation}.
We assume that the predictive ability of $\mathcal{F}$ is better than the uploaded decoders $\{\boldsymbol{\theta}_1^{dec}, \cdots, \boldsymbol{\theta}_N^{dec}\}$, and useful knowledge is primarily contained in the encoders $\{\boldsymbol{\theta}_1^{enc}, \cdots, \boldsymbol{\theta}_N^{enc}\}$. Thus, on the server side, we aim to inject medical knowledge $\{\boldsymbol{\theta}_1^{enc}, \cdots, \boldsymbol{\theta}_N^{enc}\}$ into the LLM $\mathcal{F}$ with the help of public data $\mathcal{D}_p$. Before the injection, we first aggregate knowledge uploaded from each client in a traditional federated learning manner, i.e., 
\begin{equation}
    \boldsymbol{\theta}_e = [\boldsymbol{\theta}_e^1, \cdots, \boldsymbol{\theta}_e^M] = \frac{1}{N} \sum_{n=1}^N \boldsymbol{\theta}_n^{enc}, \quad \boldsymbol{\theta}_d = [\boldsymbol{\theta}_d^1, \cdots, \boldsymbol{\theta}_d^M] = \frac{1}{N} \sum_{n=1}^N \boldsymbol{\theta}_n^{dec}.
\end{equation}


\textbf{Knowledge Injection}. 
Directly injecting medical knowledge $\boldsymbol{\theta}_e$ is challenging since the LLM $\mathcal{F}$ cannot directly use these diverse modality-specific encoders. To solve this challenge, we propose a straightforward benchmark approach that follows the training of LLaVA~\cite{liu2024visual} by concatenating the modality embeddings with the task prompt. Besides, our approach allows conducting parameter-efficient fine-tuning with the help of a designed multimodal multi-tasking mixture of experts (M$^3$OE)-based low-rank adaptation (LoRA)~\cite{hu2021lora}. Next, we detail the process of knowledge injection.

\ul{\textbf{Step 1: Feature Alignment.}}
For each input data $(\mathbf{x}_j^t, \mathbf{y}_j^t) \in \mathcal{D}_p^t$ from the $t$-th task, we first obtain its feature representations using the aggregated encoders $\boldsymbol{\theta}_e$, i.e., $\mathbf{e}_j = [\mathbf{e}_j^1; \cdots; \mathbf{e}_j^M] = g(\boldsymbol{\theta}_e(\mathbf{x}_j^t)$), where $g(\cdot)$ is the mapping function.
We also embed the task prompt $\mathcal{P}_t$ using the encoder of $\mathcal{F}$, i.e., $\mathbf{p}_t = \text{EMB}_{\mathcal{F}}(\mathcal{P}_t)$., where $\text{EMB}_\mathcal{F}()$ is the text embedding layer of $\mathcal{F}$.
Then, the concatenation of the data feature $\mathbf{e}_j$ and the task prompt feature $\mathbf{p}_t$ will be used as the input of the encoder of $\mathcal{F}$, denoted as $\mathbf{h}_j^t = [\mathbf{e}_j; \mathbf{p}_t]$.

\ul{\textbf{Step 2: Multimodal Multi-tasking Mixture of Experts (M$^3$OE).}}
A naive solution is directly using the aligned feature $\mathbf{h}_j^t$ to generate the output like LLaVA. However, such a naive end-to-end fine-tuning approach not only has weak distinguishability of different tasks but also
ignores the generalization ability of {\model} to unseen tasks, even though the modalities have been trained already. To address this issue, we develop a multimodal multi-tasking mixture of expert (M$^3$OE) modules to allow {\model} to distinguish tasks dynamically. 

M$^3$OE takes both the task description $\mathcal{T}_t$ and the modality descriptions $\mathcal{M}_m^t$ associated with Task $\mathcal{T}_t$ as inputs to compute the relevance of each expert for the given task and modality, where $\mathcal{M}_m^t$ is the concatenation of multiple modality-level descriptions. $\mathcal{T}_t$ and $\mathcal{M}_m^t$ are firstly encoded by the embedding layer of the foundation model $\mathcal{F}$, and subsequently processed to output weights for expert selection as follows:
% \begin{equation}\label{eq:refined_attention}
% \boldsymbol{\alpha}^t = \text{softmax}\left(\frac{(\mathbf{W}_q \text{EMB}_\mathcal{F}(\mathcal{M}_m)) (\mathbf{W}_k\text{EMB}_\mathcal{F}(\mathcal{T}_t))^\top}{\sqrt{d_k}}\right) \mathbf{W}_v \text{EMB}_\mathcal{F}(\mathcal{T}_t),
% \end{equation}
\begin{equation}\label{eq:refined_attention}\small
\boldsymbol{\alpha}^t=\text{softmax}\left(\text{MLP}\left(\text{Pooling}\left(\frac{(\mathbf{W}_q \text{EMB}_\mathcal{F}(\mathcal{M}_m^t)) (\mathbf{W}_k \text{EMB}_\mathcal{F}(\mathcal{T}_t))^\top}{\sqrt{d_k}}\mathbf{W}_v \text{EMB}_\mathcal{F}(\mathcal{T}_t)\right)\right)\right),  
\end{equation}
where $\boldsymbol{\alpha}^t \in \mathbb{R}^P$ and $P$ is the number of experts. $\mathbf{W}_q$, $\mathbf{W}_k$, and $\mathbf{W}_v$ denote the attention matrices, and $d_k$ is the dimension size. 




The proposed M$^3$OE effectively integrates the injected knowledge managed by two separate routers, resulting in a more streamlined and contextually aware computation of weights. The output, $\boldsymbol{\alpha}^t$, represents the attention-weighted selection of experts optimized for both the modality and the specific task. This approach provides the flexibility needed to handle complex medical scenarios by selecting the appropriate experts based on the context.

\ul{\textbf{Step 3: LoRA-M$^3$OE based Parameter-Efficient Fine-tuning.}} Finally, we generate the representation of each layer in $\mathcal{F}$ for the forward pass based on LoRA and the learned M$^3$OE weight using Eq.~\eqref{eq:refined_attention} as follows:
\begin{equation}
\mathbf{c}_j^t = \mathbf{W}_{\mathcal{F}} \mathbf{h}_j^t + \sum_{p =1}^P {\alpha}^t_p (\mathbf{B}_p \mathbf{A}_p \mathbf{h}_j^t),
\end{equation}
where $\mathbf{W}_{\mathcal{F}}$ denotes the frozen parameters of $\mathcal{F}$, 
$\mathbf{B}_p\mathbf{A}_p$ denotes the lower-rank adaptation module serving as the $p$-th expert system. We will fine-tune the proposed {\model} using the final output from $\mathcal{F}$ and the ground truth $\mathbf{y}_j^t$. 
The design balances efficacy and efficiency during knowledge injection, allowing {\model} to decently handle the complex nature of medical applications. 


During the training, modality-specific encoders $\boldsymbol{\theta}_e$ gradually align with the medical LLM $\mathcal{F}$ that contains abundant knowledge. This indicates that prior knowledge in $\mathcal{F}$ is also extracted during injection. To benefit local models and boost knowledge injection in the next round, {\model} passes the updated encoders $\boldsymbol{\theta}_e$ and the aggregated decoders $\boldsymbol{\theta}_d$ back to local ends and performs the knowledge-driven iterative training until convergence. 





==> section/problem.tex <==
\section{Problem Formulation}

% \subsection{Model Inputs}

% i-th task is denoted as $\mathbf{T}_{i}$. Each task may rely on data in multiple modlaities, denoted as $\mathcal{M}_{i} = [\mathbf{M}_{i}^0, ..., \mathbf{M}_{i}^j]$, and labels, denoted as $\mathbf{Y}_{i}$. Private data scattered in $k$-th client are denoted as $\mathbf{m}_{i,j}^{k}$ and $\mathbf{y}_{i}^{k}$, while public data stored in server are represented as $\mathbf{m}_{i,j}^{S}$.



% \subsection{Local Optimization}

% Model designed for task $\mathbf{T}_{i}$ on $k$-th client is denoted as $\mathbf{c}_{i}^{k}$. Each model consists of a feature extractor, i.e., $\text{f}_{i}^{k}$, and a predictor, i.e., $\text{p}_{i}^{k}$. Input data $\mathbf{m}_{i,j}^{k}$ are initially encoded through corresponding local modality-specific encoder, $\text{f}_{i,j}^{k}$, to obtain uniform hidden embedding $\mathbf{h}_{i,j}^{k}$ as follows:

% \begin{equation}\label{eq:local_encoding}\small
% \begin{gathered}
%  \mathbf{h}_{i,j}^{k} = \text{f}_{i,j}^{k}(\mathbf{m}_{i,j}^{k}).
% \end{gathered}
% \end{equation}

% Subsequently, we concatenate multimodal embedding for modality aggregation, i.e.,

% \begin{equation}\label{eq:local_aggregation}\small
% \begin{gathered}
%  \mathbf{h}_{i}^{k} = (\mathbf{h}_{i,1}^{k},\cdot\cdot\cdot,\mathbf{h}_{i,j}^{k}),
% \end{gathered}
% \end{equation}
% where $(\cdot, \cdot)$ denotes the concatenation operation.

% The predictor, $\text{p}_{i}^{k}$, takes $\mathbf{h}_{i}^{k}$ for making task-specific prediction, i.e.,

% \begin{equation}\label{eq:local_pred}\small
% \begin{gathered}
%  \hat{\mathbf{y}}_{i}^{k} = \text{p}_{i,j}^{k}(\mathbf{h}_{i}^{k}).
% \end{gathered}
% \end{equation}


% We locally update $\mathbf{c}_{i}^{k}$ by optimizing generative loss between ground-truth labels, $\hat{\mathbf{y}}_{i}^{k}$, and prediction, $\mathbf{y}_{i}^{k}$, i.e., 

% \begin{equation}\label{eq:local_optim}\small
% \begin{gathered}
%  \mathcal{L}_{i}^{k} = y_{i}^{k} \log(\hat{y}_{i}^{k}) + (1 - y_{i}^{k}) \log(1 - \hat{y}_{i}^{k})
% \end{gathered}
% \end{equation}

% \subsection{Communication between Client and Server}

% We produce the global model for each task through FedAVG. The encoder of global model is subsequently uploaded to the server, i.e.,

% \begin{equation}\label{eq:local_optim}\small
% \begin{gathered}
%  \mathbf{f}_{i}^{S} = \text{FedAVG}([\mathbf{f}_{i}^{0}, ..., \mathbf{f}_{i}^{K_i}])
% \end{gathered}
% \end{equation}

% where $|K_i|$ is the total number of clients for task $T_i$. The resulted module serves as the modality-specific encoder of foundation model.

% \subsection{Server Optimization}

% We propose Multi-tasking Multimodal Mixture of Experts (M3OE) to equip the foundation model with excellent capability of tackling multiple task in diverse modalities. Given specific task and corresponding modalities, a cross-attention-based router determines suitability of each expert accordingly(Section \ref{sec:MMOE}), then guides the aggregation of expert decisions (Section \ref{sec:MMOE}).




\subsection{Knowledge Injection}


% The development of an effective foundation model hinges on substantial data volumes. However, real-world medical data are highly fragmented and, due to stringent data privacy requirements, sensitive medical data cannot be freely distributed. This situation results in a limited amount of public data available, which hampers the centralized development of medical foundation models. We articulate this challenge as follows:

% The development of an effective foundation model hinges on substantial data volumes. Nevertheless, due to privacy constraints, most medical data are preserved within individual clinical institutions. These scattered datasets can only be leveraged by lightweight models distributed across different clients, and cannot be directly accessed by the centralized medical foundation model. In such cases, medical knowledge, rather than raw data, becomes the intermediary passed from clients to the foundation model deployed on the server. This approach ensures that sensitive patient information remains secure while still enhancing the medical foundation model through shared knowledge. 

% However, the nature of medical data—being noisy, multimodal, and temporally complex—makes knowledge injection challenging, as unsuitable injection might not effectively boost the foundation model. Therefore, appropriately injecting knowledge into the model becomes crucial to support the development and efficacy of the medical foundation model.

% We propose three important stages during the whole process of medical knowledge injection:

% \noindent\textbf{Knowledge Extraction.} Effectively extracting high-quality medical knowledge from distributed models and scattered datasets is crucial. The accuracy and relevance of the distilled knowledge directly impact whether the foundation model gains valuable insights or merely noise. Ensuring the precision of this extraction process is vital for the overall performance of the model.

% \noindent\textbf{Knowledge Transfer.} Transferring the extracted medical knowledge to the foundation model is an ongoing challenge. This process involves not only the physical transfer of data but also the integration of knowledge in a way that the model can utilize it effectively. Addressing the complexities of this transfer is essential for the seamless enhancement of the model.

% \noindent\textbf{Knowledge Interiorization.} Even after extraction and transfer, external knowledge may not be immediately usable by the foundation model. Proper accommodation is necessary to embed this external knowledge into the medical foundation model effectively. This step ensures that the integrated knowledge aligns with the model's structure and enhances its capabilities.



We conceptualize the ultimate objective of medical knowledge injection through federated learning as follows: \textbf{The centralized Medical Foundation Model (MFM), initially limited by its access to data, is enriched by leveraging distributed client models that benefit from a wide range of scattered data, thereby enabled to gain from the diverse knowledge of these smaller models after communication}. This enrichment enables the MFM to better address new modalities and undertake previously unseen tasks. Let us denote the Medical Foundation Model as $\mathbf{F}$ and the localized, specialized models as $\mathcal{L}$, where $\mathcal{L}$ consists of an array of models such as $\mathcal{L} = [\mathbf{L_{1}}, \ldots, \mathbf{L_{i}}]$, each highly specialized for distinct modalities and tasks. The modality handled by a model is represented as $M(\cdot)$, and the task addressed by a model is denoted as $T(\cdot)$. The problem of medical knowledge injection can be mathematically formulated as follows:
Prior to the injection, the foundation model is restricted by its pre-trained domain and modalities, thus only capable of addressing a narrow range of modalities and tasks, i.e., 
\begin{equation}
% \begin{split}
    M(\mathbf{F}) << \bigcup_{i \in |\mathcal{L}|} M(\mathbf{L}_i), 
    T(\mathbf{F}) << \bigcup_{i \in |\mathcal{L}|} T(\mathbf{L}_i).
% \end{split}
\end{equation}

Following the injection, the foundation model is enhanced to effectively handle previously unseen modalities and tasks, broadening its applicative scope, i.e., 

\begin{equation}
% \begin{split}
    M(\mathbf{F}) = \bigcup_{i \in |\mathcal{L}|} M(\mathbf{L}_i), 
    T(\mathbf{F}) = \bigcup_{i \in |\mathcal{L}|} T(\mathbf{L}_i).
% \end{split}
\end{equation}

\subsubsection{Knowledge Extraction}

\subsubsection{Knowledge Transfer}

\subsubsection{Knowledge  Interiorization}


% \subsection{Data Distribution}

% Developing an effective foundation model proposed demand on volume of data. However, real-world medical data are highly scattered. Due to intensive requirement on data privacy, sensitive medical data cannot be causally distributed. This nature results in limited amount of public data available for accessing, impeding the centralized development of medical foundation model. We formulate this problem as follows:


% \subsection{{\model}: An Initial Solution}

% To handle this unsolved yet essential problem, we propose our solution, i.e., {\model}, as the benchmark on this problem. {\model} is designed to solve two key questions in the development of Medical Foundation Model, i.e., how to convey the knowledge to the model, and how to urge the model to interiorizes the delivered knowledge. {\model} applies the Federated Encoding strategy (Section \ref{sec:fed}) to handle the former challenge, and the Multi-tasking Multimodal Mixture of Experts (Section \ref{sec:MMOE}) to tackle the latter concern.
    


\subsection{{\model}: An Initial Solution}

\xiaochen{A figure here.} Addressing this critical yet unresolved issue, we introduce {\model} as a pioneering benchmark for this challenge. {\model} is engineered to answer two fundamental questions in the development of a Medical Foundation Model: how to effectively transfer knowledge to the model, and how to ensure the model assimilates this imparted knowledge. To address these, {\model} adopts Lora-MoE approach for Parameter-efficient fine-tuning, employs a Federated Encoding strategy
% (Section \ref{sec:fed}) 
to facilitate knowledge transfer, and utilizes a Multi-tasking Multimodal Mixture of Experts approach 
% (Section \ref{sec:MMOE})
to enhance knowledge assimilation.




% \subsubsection{Federated Encoding}
% \label{sec:fed}

\noindent\textbf{Knowledge Extraction.} {\model} deploys local models to clients for knowledge extraction. Local models are trained on scattered private data, optimized by Cross Entropy loss. These models are aggregated through FedAVG, producing an global model containing knowledge gathered from diverse sources of private data.
% % Initialization
% Initialize $\mathbf{w}_0$.

% % For each round
% For each round $t = 0, 1, 2, \ldots$:
% \begin{enumerate}
%     \item Server sends $\mathbf{w}_t$ to all clients.
%     \item Each client $k$ updates its local model parameters:
%     \begin{equation}
%         \mathbf{L}_k^{t+1} = \mathbf{w}_t - \eta \nabla \ell(\mathbf{w}_t; D_k)
%     \end{equation}
%     \item Server aggregates the updated parameters:
%     \begin{equation}
%         \mathbf{w}_{t+1} = \sum_{k=1}^K \frac{|D_k|}{\sum_{j=1}^K |D_j|} \mathbf{L}_k^{t+1}
%     \end{equation}
% \end{enumerate}


\xiaochen{Will modify tomorrow to only introduce the parameter sharing.}
\noindent\textbf{Knowledge Transfer.} Promising medical foundation models are expected to handle a wide spectrum of modalities. While conventional medical foundation models \cite{} only tackle fewer than two modalities, {\model} is designed to handle an arbitrary number of modalities. For each modality, {\model} utilizes a modality-specific encoder to embed external tokens into the semantic space of the backbone LLM. The input of {\model}, denoted as $\mathbf{X}$, consists of a sequence of embeddings produced by the corresponding encoders, i.e.,

\begin{equation}
\mathbf{X} = \left[ \mathbf{E}_1(\mathbf{x}_1), \mathbf{E}_2(\mathbf{x}_2), \ldots, \mathbf{E}_n(\mathbf{x}_n) \right],
\end{equation}
where $[\cdot,\cdot]$ denotes the concatenation operation, $x_{i}$ denotes $i-th$ modality, and $E_{i}$ denotes corresponding encoder. In each communication round, $E_{i}$ are distributed to multiple local clients, optimized on local data, and produced an aggregated encoder through Federated Average. \xiaochen{See if we can try different ones}. 

Although the aggregated encoder benefits enough from the federated optimization, its produced feature cannot be directly internalized by the foundation model, as the feature distribution might be shifted beyond the domain of definition of foundation model. Therefore,after taking parameters uploaded from clients for updating its modality-specific encoder, the foundation model further align external encoder and local weights through optimization on server data.

Details on optimization can be found in the Appendix.







% \subsubsection{Multi-tasking Multimodal Mixture of Experts}
% \label{sec:MMOE}


\noindent\textbf{Multi-tasking Multimodal Mixture of Experts} Flexibly handling different tasks and modalities with complex combinations, although promising for a medical foundation model, is still challenging. To tackle the challenge, we propose using a single attention-based mechanism to dynamically generate the weights for selecting the most suitable experts. The attention mechanism takes both the modality description $\textit{M}$ and the task description $\textit{T}$ as inputs to compute the relevance of each expert for the given task and modality. The descriptions firstly encoded by embedding layer of foundation model, subsequently processed to output weights for expert selection as follows:

\begin{equation}\label{eq:refined_attention}\small
\begin{gathered}
\mathbf{w}_{i} = \text{softmax}\left(\frac{(\mathbf{W}_q \mathbf{m}) (\mathbf{W}_k\mathbf{t})^T}{\sqrt{d_k}}\right) \mathbf{W}_v \mathbf{t},\\
\mathbf{m} = \mathbf{W_e} \cdot \textit{M},\\
\mathbf{t} = \mathbf{W_e} \cdot \textit{T},
\end{gathered}
\end{equation}
where $\mathbf{W_e}$ denotes the embedding layer of foundation model. 

This single attention mechanism effectively integrates the information previously managed by two separate routers, resulting in a more streamlined and contextually aware computation of weights. The output, $\mathbf{w_{i}}$, represents the attention-weighted selection of experts, optimized for both the modality and the specific task. By selecting the appropriate experts based on the context, this approach provides the flexibility needed to handle complex medical scenarios.


Given the context of modalities and tasks, the Lora-MOE is optimized as follows:

\begin{equation}
\mathbf{Y}_{\text{LoRA-MoE}} = \mathbf{W}_{\text{original}} \mathbf{X} + \sum_{i \in \mathcal{E}} \mathbf{w}_{i} (\mathbf{A}_i \mathbf{B}_i \mathbf{X}),
\end{equation}

where $\mathbf{W}_{\text{original}}$ denotes the backbone foundation model, $\mathbf{A}_i \mathbf{B}_i$ denotes the lower-rank adaptation module serving as $i$-th expert system.






==> section/problem_new.tex <==
\section{Problem Formulation}

\subsection{Preliminaries}

% Healthcare tasks are denoted as $\mathcal{T} = [\text{T}_0, ..., \text{T}_i]$. Suite of modalities available in the domain of healthcare are denoted as $\mathcal{M} = [\text{M}_0, ..., \text{M}_i]$. 
% Features in modality $\text{M}_j$ used to solve task $\text{T}_i$ are denoted as $\text{x}_{i,j}$, while ground-truth labels for task $\text{T}_i$ are denoted as $\text{y}_{i}$. 

% Private data scattered in $k$-th institution are denoted as $\text{x}_{i,j}^{k}$ and $\text{y}_{j}$, while public data accessible to foundation model are represented as $\text{d}_{i,j}^{P}$ and $\text{y}_{j}$. 

 
%  Each institution, although limited by computing resource, are still capable to tackle diverse healthcare modalities in the context to multiple tasks. Therefore, we assume $k$-th healthcare institution possesses a multi-task mutlimodal model, denoted as $\mathbf{l}_{k}$. For each modality $\mathbf{M_j}$, $\mathbf{l}_{k}$ own a modality-specific encoder, denoted as $\text{e}_{j}^{k}$. To handle all the modality and tasks, $\mathbf{l}_{k}$ consists of encoders whose number equals with the amount of modality. Similarly, $\mathbf{l}_{k}$ owns task-specific heads for making prediction on each individual healthcare task, denoted as $\text{p}_{i}^{k}$. The number of task-specific heads equals to the amount of clinical tasks, meaning that $\mathbf{l}_{k}$ is capable of handling all the healthcare task, regardless of its capability. Therefore, for an arbitrary task, $\mathbf{l}_{k}$ takes features in all relevant modalities as input, and make the prediction as follows:

 Healthcare tasks are denoted as $\mathcal{T} = [\text{T}_0, \ldots, \text{T}_i]$. The suite of modalities available in the domain of healthcare are denoted as $\mathcal{M} = [\text{M}_0, \ldots, \text{M}_j]$. Features in modality $\text{M}_j$ used to solve task $\text{T}_i$ are denoted as $\text{x}_{i,j}$, while ground-truth labels for task $\text{T}_i$ are denoted as $\text{y}_i$.

Private data scattered across the $k$-th institution are denoted as $\textbf{x}_{i,j}^{k}$ and $\textbf{y}_i^{k}$, while public data accessible to the foundation model are represented as $\textbf{x}_{i,j}^{P}$ and $\textbf{y}_i^{P}$.






Foundation model deployed on the server is denoted as $\text{F}$. Each institution, although limited by computing resources, is capable of handling diverse healthcare modalities in the context of multiple tasks. Therefore, we assume the $k$-th healthcare institution possesses a multi-task multimodal model, denoted as $\text{l}_k$.

For each modality $\text{M}_j$, $\text{l}_k$ has a modality-specific encoder, denoted as $\text{e}_{j}^{k}$. To handle all modalities and tasks, $\text{l}_k$ consists of encoders equal in number to the modalities. Similarly, $\text{l}_k$ owns task-specific heads for making predictions on each individual healthcare task, denoted as $\text{p}_{i}^{k}$. The number of task-specific heads equals the number of clinical tasks, meaning that $\text{l}_k$ is capable of handling all healthcare tasks, regardless of its capability. Therefore, for an arbitrary task $\text{T}_i$, $\text{l}_k$ takes features from all relevant modalities as input and makes the prediction as follows:

\newcommand{\concat}{\mathcal{C}}

\begin{equation}\label{eq:local_encoding}
\small
\begin{gathered}
 \hat{\mathbf{y}}_{i}^{k} = \text{p}_{i}^{k}(\concat_{j=1}^{m} \text{e}_{j}^{k}(\text{x}_{i,j}^{k}))
\end{gathered}
\end{equation}

where $\concat_{j=1}^{m}$ represents concatenation of the embeddings from all modalities $M_j$. The design of local model $\text{l}_k$ ensures its flexibility, allowing it to serve as not only a counterpart but also a component in our proposed {\model}, introduced undermentioned.










% \begin{equation}\label{eq:local_encoding}
% \begin{gathered}
%  \hat{\mathbf{y}}_{i} = \text{p}_{i}^{k}([\text{e}_{1}^{k}(\mathbf{x}_{i,1}^{k}), \text{e}_{2}^{k}(\mathbf{x}_{i,2}^{k}), \ldots, \text{e}_{m}^{k}(\mathbf{x}_{i,m}^{k})])
% \end{gathered}
% \end{equation}


 
 
%  Model designed for task $\mathbf{T}_{i}$ on $k$-th client is denoted as $\mathbf{c}_{i}^{k}$. Each model consists of an encoder, i.e., $\text{e}_{i}^{k}$, and a predictor, i.e., $\text{p}_{i}^{k}$. Input data $\mathbf{m}_{i,j}^{k}$ are initially encoded through corresponding local modality-specific encoder, $\text{e}_{i,j}^{k}$, to obtain uniform hidden embedding $\mathbf{h}_{i,j}^{k}$ as follows:

% \begin{equation}\label{eq:local_encoding}\small
% \begin{gathered}
%  \mathbf{h}_{i,j}^{k} = \text{f}_{i,j}^{k}(\mathbf{m}_{i,j}^{k}).
% \end{gathered}
% \end{equation}

\subsection{{\model}: An Intial Solution}
% \xiaochen{A figure here.} Addressing this critical yet unresolved issue, we introduce {\model} as a pioneering benchmark for this challenge. {\model} is engineered to answer two fundamental questions in the development of a Medical Foundation Model: how to effectively transfer knowledge to the model, and how to ensure the model assimilates this imparted knowledge. To address these, {\model} adopts Lora-MoE approach for Parameter-efficient fine-tuning, employs a Federated Encoding strategy
% % (Section \ref{sec:fed}) 
% to facilitate knowledge transfer, and utilizes a Multi-tasking Multimodal Mixture of Experts approach 
% % (Section \ref{sec:MMOE})
% to enhance knowledge assimilation.

The medical knowledge injection problem, though necessary, has not been adequately addressed in previous research. The absence of a standardized benchmark has hindered researchers from exploring this valuable topic. To fill this gap, we introduce {\model}, a pioneering benchmark designed to tackle this challenge. {\model} is engineered to perform knowledge injection following the aforementioned three stages: knowledge extraction (Sec. \ref{sec:knowledge_extraction}), knowledge transfer (Sec. \ref{sec:knowledge_transfer}), and knowledge interiorization (Sec. \ref{sec:knowledge_interiorization}).


\subsection{Knowledge Extraction}
\label{sec:knowledge_extraction}

The privacy issue, as mentioned in \ref{sec:intro}, significantly impedes foundation model to benefit from large amount of private data. Therefore, the only possible method is to obtain a type of knowledge by leveraging scattered data, then deliver the knowledge to the foundation model. 

Here, we define the knowledge as well-learned parameters on the local model that safe to share without privacy issue. For obtaining local knowledge effectively, {\model} applies a multi-tasking multimodal optimization strategy along with Cross Entropy, described as follows:

\begin{equation}\label{eq:client_loss}
\mathcal{L}_{k} =  \sum_{i} ( y_{i}^{k} \log(\hat{y}_{i}^{k}) + (1 - y_{i}^{k}) \log(1 - \hat{y}_{i}^{k}) ).
\end{equation}

This objective function allows the local model to benefit from all modalities and tasks relevant to this client, thus optimizing all the modality-specific encoders and task-specific head. Thus, the local models are equipped with decent ability of knowledge extraction, assuring the quality of knowledge further transferred to foundation model \text{F}.



\subsection{Knowledge Transfer}
\label{sec:knowledge_transfer}
Although knowledge have been effectively extracted as aforementioned, the knowledge is still scattered, contained in local models in different healthcare institutions. Without appropriate method, the distributed knowledge cannot be directly applied to the foundation model. To handle this challenge, we apply FedAvg for producing knowledge-rich encoders by aggregating the distributed modality-specific encoders as follows:




\begin{equation}
\text{e}_{j} = \frac{1}{K} \sum_{k=1}^{K} \text{e}_{j}^{k},
\end{equation}

where $K$ is the number of clients. Through the federated learning approach, we obtain well-trained encoders for each modalities. Subsequently, The encoders are sent to the foundation model deployed on the server end. Equipped with these knowledge-rich encoders, the foundation model, previously limited for handling wide spectrum of modalities, are now able to tackle these valuable healthcare information.






The aggregated encoder then serves as encoder for the medical foundation model, transferring knowledge extracted from scattered medical data into the foundation model.

\subsection{Knowledge Interiorization}
\label{sec:knowledge_interiorization}


After the knowledge extraction and trasnfer, the foundation model \text{F}, are enabled with multimodal capability. However, these knowledge-rich encoders are externally optimized, meaning that knowledge preserved in their weights may not be directly used by the foundation model. Although their generated embeddings are informative, they are out of the domain of foundation model. Without appropriate alignment between external encoders and foundation model, the knowledge cannot be appropriate used, and might even result in noise introduction. Therefore, encouraging the foundation model to interiorize knowledge is a necessary stage. To achieve that, we leverage the public data, $\textbf{x}_{i,j}^{P}$ and $\textbf{y}_i^{P}$, for establishing alignmented between external and internal knowledge. 


For an arbitrary task $\text{T}_i$, the foundation model $\text{F}$ takes public data in corresponding modalities, i.e., $\bigcup_{j} \text{x}_{i,j}^{P}$, as input. The foundation model, empowered by the knowledge-rich encoders, is now enabled to transform the heterogeneous healthcare modalities into unified form of embeddings, i.e., 

\begin{equation}\label{eq:concatenated_encoding}
\small
\begin{gathered}
\mathbf{h}_i = \concat_{j=1}^{n} \text{e}_{j}(\mathbf{x}_{i, j}^P),
\end{gathered}
\end{equation}


where $\concat$ denotes the concatenation. The unification on diverse input modalities eliminates the heterogeneity of healthcare data, serving as the prerequisite of integrating external knowledge. Later, we propose the Multi-tasking Multimodal Mixture of Experts (M3OE) to effectively absorb external knowledge through well-designed guidance. 




% \subsubsection{Multi-tasking Multimodal Mixture of Experts}
% \label{sec:MMOE}


\noindent\textbf{Multi-tasking Multimodal Mixture of Experts} Inputs of {\model} derives from various modalities and resources. Flexibly handling different tasks and modalities with complex combinations, although promising for a medical foundation model, is still challenging. To tackle the challenge, we propose using an attention-based mechanism to dynamically generate the weights for selecting the most suitable experts. The attention mechanism takes both the modality description $\textit{M}$ and the task description $\textit{T}$ as inputs to compute the relevance of each expert for the given task and modality. The descriptions firstly encoded by embedding layer of foundation model, subsequently processed to output weights for expert selection as follows:

\begin{equation}\label{eq:refined_attention}\small
\begin{gathered}
\mathbf{w} = \text{softmax}\left(\frac{(\mathbf{W}_q \mathbf{m}) (\mathbf{W}_k\mathbf{t})^T}{\sqrt{d_k}}\right) \mathbf{W}_v \mathbf{t},\\
\mathbf{m} = \mathbf{W}_e \cdot \textit{M},\\
\mathbf{t} = \mathbf{W}_e \cdot \textit{T},
\end{gathered}
\end{equation}
where $\mathbf{W}_q$, $\mathbf{W}_k$, $\mathbf{W}_v$ denotes the attention matrices, $\mathbf{W}_e$ denotes the embedding layer of foundation model. 

This attention mechanism effectively integrates the injected knowledge managed by two separate routers, resulting in a more streamlined and contextually aware computation of weights. The output, $\mathbf{w_{i}}$, represents the attention-weighted selection of experts, optimized for both the modality and the specific task. By selecting the appropriate experts based on the context, this approach provides the flexibility needed to handle complex medical scenarios.


Given the context of modalities and tasks, the Lora-MOE is optimized as follows:

\begin{equation}
\hat{\mathbf{Y}} = \mathbf{W}_{\text{F}} \mathbf{h}_i + \sum_{p \in \mathcal{P}} \mathbf{w}_{i} (\mathbf{A}_i \mathbf{B}_i \mathbf{h}_i),
\end{equation}

where $\mathbf{W}_{\text{F}}$ denotes the backbone foundation model parameters, $\mathbf{A}_p \mathbf{B}_p$ denotes the lower-rank adaptation module serving as $p$-th expert system. The design balance efficacy and efficiency during knowledge interiorization, allowing {\model} to decently handle the complex nature of medical applications. 


uring the training, modality-specific encoders gradually align with foundation model $\text{F}$ that contains abundant knowledge. This indicates that prior knowledge in foundation model is also extracted during the interiorization process. To benefit local models and boost knowledge injection in the next round, {\model} passes encoders back to local ends, and performs the knowledge-driven iterative training until converge. 




==> section/task.tex <==
\section{Dataset \& Task}

The medical foundation model, as emphasized in \cite{moor2023foundation}, should be capable of handling multiple tasks across diverse modalities. Accordingly, this benchmark encompasses a wide spectrum of tasks involving various medical modalities in flexible combinations, reflecting the complex scenarios that the medical foundation model is expected to address. The tasks, modalities, and datasets involved in this study are listed in Figure \ref{}. 
% \ref{tab:datasets}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{fig/data_tasks_modality.png}
    \caption{Representative healthcare modality, tasks and datasets covered in this study.}
    \label{fig:data}
   % \vspace{-0.1in}
\end{figure}


% \begin{table}[]
% \tiny
% \begin{tabular}{l|l|l|l|llll}
% \hline
% Task Type                                              & Modality                                   & Task                                  & Dataset   & \# of Total Samples & \# of Training Samples on Clients & \# of Training Samples on Server & \# of Test Samples \\ \hline
% \multirow{10}{*}{Unimodal Task}                        & \multirow{3}{*}{Image}                     & Image Classification                      & RSNA      &                     &                                   &                                  &                    \\ \cline{3-8} 
%                                                        &                                            & Covid Detection                           & Covid-19  &                     &                                   &                                  &                    \\ \cline{3-8} 
%                                                        &                                            & Cardiomediastinum Prediction              & CheXpert  &                     &                                   &                                  &                    \\ \cline{2-8} 
%                                                        & \multirow{2}{*}{Text}                      & ICD Coding                                & MIMIC-III &                     &                                   &                                  &                    \\ \cline{3-8} 
%                                                        &                                            & MedQA                                     & MedQA     &                     &                                   &                                  &                    \\ \cline{2-8} 

%                                                        & \multirow{2}{*}{Audio}                     & \multirow{2}{*}{Covid Detection}          & CoughVID  &                     &                                   &                                  &                    \\ \cline{4-8} 
%                                                        &                                            &                                           & DICOVA    &                     &                                   &                                  &                    \\ \cline{2-8} 
%                                                        & \multirow{2}{*}{ECG}                       & \multirow{2}{*}{Sleep Apnea Detection}    & MIT-BIH   &                     &                                   &                                  &                    \\ \cline{4-8} 
%                                                        &                                            &                                           & Apnea ECG &                     &                                   &                                  &                    \\ \hline
% \multicolumn{1}{c|}{\multirow{10}{*}{Multimodal Task}} & \multirow{6}{*}{Temporal Readings, Demographics} & \multirow{2}{*}{ARF Prediction}           & MIMIC-III &                     &                                   &                                  &                    \\ \cline{4-8} 
% \multicolumn{1}{c|}{}                                  &                                            &                                           & eICU      &                     &                                   &                                  &                    \\ \cline{3-8} 
% \multicolumn{1}{c|}{}                                  &                                            & \multirow{2}{*}{Shock Prediction}         & MIMIC-III &                     &                                   &                                  &                    \\ \cline{4-8} 
% \multicolumn{1}{c|}{}                                  &                                            &                                           & eICU      &                     &                                   &                                  &                    \\ \cline{3-8} 
% \multicolumn{1}{c|}{}                                  &                                            & \multirow{2}{*}{Mortality Prediction (valid)}     & MIMIC-III &                     &                                   &                                  &                    \\ \cline{4-8} 
% \multicolumn{1}{c|}{}                                  &                                            &                                           & eICU      &                     &                                   &                                  &                    \\ \cline{2-8} 
% \multicolumn{1}{c|}{}                                  & \multirow{4}{*}{Text, Image}               & \multirow{2}{*}{MedVQA (valid)}                   & RAD       &                     &                                   &                                  &                    \\ \cline{4-8} 
% \multicolumn{1}{c|}{}                                  &                                            &                                           & Slake     &                     &                                   &                                  &                    \\ \cline{3-8} 
% \multicolumn{1}{c|}{}                                  &                                            & \multirow{2}{*}{Medical Image Captioning} & CheXpert &                     &                                   &                                  &                    \\ \cline{4-8} 
% \multicolumn{1}{c|}{}                                  &                                            &                                           & Openl     &                     &                                   &                                  &                    \\ \cline{2-8}
% \multicolumn{1}{c|}{}                                  & ECG, Text                                          &  \multirow{1}{*}{ECG QA}                                          & ECG-QA     &                     &                                   &                                  &                    \\ \hline
% \end{tabular}
% \caption{Tasks, modalities and datasets involved in this study.}
% \label{tab:datasets}
% \end{table}


\begin{table}[]
\small
\begin{tabular}{l|l|l|l}
\hline
Task Type                                              & Modality                                   & Task                                  & Dataset   \\ \hline
\multirow{8}{*}{Unimodal Task}                        & \multirow{3}{*}{Image}                     & Lung Opacity Detection                & RSNA      \\ \cline{3-4} 
                                                       &                                            & Covid Detection                       & Covid-19  \\ \cline{3-4} 
                                                       &                                            & Cardiomediastinum Prediction          & CheXpert  \\ \cline{2-4} 
                                                       & Text                                       & MedQA                                 & MedQA     \\ \cline{2-4} 
                                                       & Signal                                     & Sleep Apnea Detection                 & MIT-BIH   \\ \cline{2-4} 
                                                       & Temporal Clinical Readings                 & ARF Prediction                        & MIMIC-III \\ \cline{3-4} 
                                                       &                                            & Shock Prediction                      & MIMIC-III \\ \cline{3-4} 
                                                       &                                            & Mortality Prediction                  & MIMIC-III \\ \hline
\multirow{2}{*}{Multimodal Task}                       & Text, Image                                & MedVQA                                & RAD       \\ \cline{2-4} 
                                                       & Signal, Text                               & Signal QA                             & ECG-QA    \\ \hline
\end{tabular}
\caption{Tasks, modalities and datasets involved in this study.}
\label{tab:datasets}
\end{table}



% \begin{table}[]
% \tiny
% \begin{tabular}{l|l|l|l|llll}
% \hline
% Task Type                                              & Modality                                   & Task                                  & Dataset   & \# of Total Samples & \# of Training Samples on Clients & \# of Training Samples on Server & \# of Test Samples \\ \hline
% \multirow{3}{*}{Unimodal Task}                        & \multirow{1}{*}{Image}                     & Lung Opacity Detection                      & RSNA      &                     &                                   &                                  &                    \\ \cline{2-8} 
                                       
%                                                        & \multirow{1}{*}{Text}                      & MedQA                                     & MedQA     &                     &                                   &                                  &                    \\ \cline{2-8} 

                                                      
%                                                        & \multirow{1}{*}{Signal}                       & \multirow{1}{*}{Sleep Apnea Detection}    & MIT-BIH   &                     &                                   &                                  &                    \\ \hline
% \multicolumn{1}{c|}{\multirow{3}{*}{Multimodal Task}} & \multirow{2}{*}{Temporal Readings, Demographics} & \multirow{1}{*}{ARF Prediction}           & MIMIC-III &                     &                                   &                                  &                    \\ \cline{3-8} 
% \multicolumn{1}{c|}{}                                  &                                            & \multirow{1}{*}{Shock Prediction}         & MIMIC-III &                     &                                   &                                  &                    \\ \cline{2-8} 
% \multicolumn{1}{c|}{}                                  & \multirow{1}{*}{Text, Image}               & \multirow{1}{*}{MedVQA (valid)}                   & RAD       &                     &                                   &                                  &                    \\ \cline{2-8} 
% \multicolumn{1}{c|}{}                                  & ECG, Text                                          &  \multirow{1}{*}{ECG QA}                                          & ECG-QA (valid)    &                     &                                   &                                  &                    \\ \hline
% \end{tabular}
% \caption{Tasks, modalities and datasets involved in this study.}
% \label{tab:datasets}
% \end{table}

==> section/task_new.tex <==
\section{Medical Modalities, Tasks and Datasets}
Medical data are significantly more complex compared to data in general domains such as computer vision and natural language processing. Common modalities in medical data include patient demographics, medical records, lab test results, vital signs, images, treatment plans, and clinical notes. However, due to health regulations like the Health Insurance Portability and Accountability Act (HIPAA) in the USA, accessing all these modalities simultaneously for model training is often impossible.

Current publicly available medical datasets typically contain only a subset of these modalities. Researchers build predictive models based on the available modalities, which can be categorized into unimodal and multimodal tasks. Unimodal tasks use specific modality data, such as medical images or continuous monitoring signals, to make predictions about certain diseases. Conversely, multimodal tasks utilize multiple modalities, learning the interactions among them to achieve predictions or answer questions.

In this work, we will explore XXX medical modalities and XXX medical tasks, extracted from XXX publicly available datasets. A summary of the modalities, tasks, and datasets can be found in Figure~\ref{XXX}.
